The DLV System for Knowledge Representation and Reasoning

This paper presents the DLV system, which is widely considered the state-of-the-art implementation of disjunctive logic programming, and addresses several aspects. As for problem solving, we provide a formal definition of its kernel language, function-free disjunctive logic programs (also known as disjunctive datalog), extended by weak constraints, which are a powerful tool to express optimization problems. We then illustrate the usage of DLV as a tool for knowledge representation and reasoning, describing a new declarative programming methodology which allows one to encode complex problems (up to $\Delta^P_3$-complete problems) in a declarative fashion. On the foundational side, we provide a detailed analysis of the computational complexity of the language of DLV, and by deriving new complexity results we chart a complete picture of the complexity of this language and important fragments thereof. Furthermore, we illustrate the general architecture of the DLV system which has been influenced by these results. As for applications, we overview application front-ends which have been developed on top of DLV to solve specific knowledge representation tasks, and we briefly describe the main international projects investigating the potential of the system for industrial exploitation. Finally, we report about thorough experimentation and benchmarking, which has been carried out to assess the efficiency of the system. The experimental results confirm the solidity of DLV and highlight its potential for emerging application areas like knowledge management and information integration.

==> sokoban-table <==
1 & 15.41 & - & - & - & 75.13 & 23.78 & 6.36\\
2 & 0.16 & - & - & - & 0.71 & 0.61 & 0.80\\
3 & 0.21 & - & - & - & 1.12 & 0.88 & 0.97\\
4 & 0.13 & 55.71 & 49.05 & 58.36 & 0.69 & 0.58 & 0.75\\
5 & 0.32 & - & - & - & 1.53 & 1.25 & 1.73\\
6 & 0.11 & 34.49 & 30.43 & 32.40 & 0.48 & 0.42 & 0.53\\
7 & 0.15 & 84.43 & 74.44 & 70.66 & 0.77 & 0.62 & 0.75\\
8 & 0.46 & - & - & - & 2.13 & 1.74 & 2.00\\
9 & 0.09 & - & 99.32 & 94.25 & 0.43 & 0.36 & 0.43\\
10 & 0.18 & - & - & - & 0.84 & 0.69 & 0.79\\
11 & 0.15 & - & 155.04 & 145.69 & 0.69 & 0.58 & 0.69\\
12 & 0.17 & - & 156.24 & 186.24 & 0.80 & 0.68 & 0.80\\
13 & 0.06 & 13.20 & 11.52 & 11.34 & 0.33 & 0.28 & 0.35\\
14 & 0.11 & 34.54 & 30.47 & 32.04 & 0.58 & 0.48 & 0.57\\
15 & 0.17 & - & - & - & 0.81 & 0.68 & 0.84\\
16 & 1.14 & - & - & - & 5.69 & 4.09 & 4.41\\
17 & 0.14 & - & 109.28 & 119.88 & 0.71 & 0.58 & 0.71\\
18 & 0.92 & - & - & - & 5.72 & 3.68 & 3.08\\
19 & 0.59 & - & - & - & 5.20 & 3.22 & 2.87\\
20 & 0.76 & - & - & - & 4.48 & 3.19 & 2.73\\
21 & 0.27 & - & 157.43 & 162.44 & 1.23 & 1.01 & 1.16\\
22 & 0.27 & - & 223.57 & 209.98 & 1.18 & 0.98 & 1.11\\
23 & 0.29 & - & 224.04 & - & 1.34 & 1.07 & 1.45\\
24 & 0.26 & - & 157.67 & 170.00 & 1.24 & 1.00 & 1.33\\
25 & 0.08 & 11.35 & 9.91 & 10.72 & 0.43 & 0.36 & 0.47\\
26 & 0.38 & - & 213.14 & 248.01 & 1.94 & 1.56 & 1.93\\
27 & 0.06 & 13.26 & 11.58 & 11.23 & 0.32 & 0.27 & 0.36\\
28 & 0.34 & - & - & - & 1.51 & 1.20 & 1.55\\
29 & 0.54 & - & 191.14 & 241.92 & 3.14 & 2.28 & 2.66\\
30 & 0.39 & - & - & - & 1.66 & 1.32 & 1.52\\
31 & 0.53 & - & - & - & 2.74 & 1.89 & 2.12\\
32 & 0.06 & 13.41 & 11.69 & 12.74 & 0.35 & 0.29 & 0.37\\
33 & 0.31 & - & - & - & 1.46 & 1.20 & 1.46\\
34 & 0.49 & - & - & - & 1.96 & 1.59 & 1.99\\
35 & 1.00 & - & - & - & 4.71 & 3.27 & 4.06\\
36 & 0.20 & 79.70 & 70.27 & 77.99 & 1.02 & 0.83 & 1.08\\
37 & 0.66 & - & - & - & 3.07 & 2.33 & 2.26\\
38 & 0.46 & - & 215.15 & 271.75 & 2.04 & 1.61 & 2.08\\
39 & 0.43 & - & - & - & 1.87 & 1.49 & 2.03\\
40 & 0.27 & - & 157.08 & 181.74 & 1.19 & 0.99 & 1.37\\
41 & 0.32 & - & 145.70 & 153.56 & 1.56 & 1.26 & 1.55\\
42 & 0.31 & 107.89 & 95.94 & 109.38 & 1.48 & 1.22 & 1.52\\
43 & 0.74 & - & - & - & 4.07 & 2.88 & 2.82\\
44 & 0.38 & - & 214.17 & 224.76 & 1.64 & 1.34 & 1.58\\
45 & 0.49 & - & 191.05 & 218.84 & 2.32 & 1.88 & 2.19\\
46 & 0.69 & - & 353.98 & - & 4.05 & 2.78 & 3.77\\
47 & 0.96 & - & - & - & 5.36 & 3.32 & 3.24\\
48 & 0.89 & - & 354.23 & - & 4.17 & 3.06 & 3.38\\
49 & 0.41 & - & - & - & 1.85 & 1.52 & 1.63\\
50 & 659.02 & - & - & - & 233.07 & 370.21 & 12.00\\
51 & 198.84 & - & - & - & - & 2033.88 & 263.88\\
52 & - & - & - & - & - & 5631.03 & 234.42\\
53 & 0.56 & - & 279.91 & 322.20 & 3.32 & 2.40 & 2.71\\
54 & 12.31 & - & - & - & 163.51 & 45.96 & 13.00\\
55 & 320.44 & - & - & - & 196.89 & 122.37 & 129.66\\
56 & 2.70 & - & - & - & 13.08 & 6.86 & 6.65\\
57 & - & - & - & - & - & - & -\\
58 & - & - & - & - & - & - & -\\
59 & 19.98 & - & - & - & 106.95 & 104.58 & 19.55\\
60 & 5.27 & - & - & - & 173.32 & 25.65 & 19.32\\

